Distributed Complexity of $P_k$-freeness: Decision and Certification

The class of graphs that do not contain a path on $k$ nodes as an induced subgraph ($P_k$-free graphs) has rich applications in the theory of graph algorithms. This paper explores the problem of deciding $P_k$-freeness from the viewpoint of distributed computing. For specific small values of $k$, we present the \textit{first} $\mathsf{CONGEST}$ algorithms specified for $P_k$-freeness, utilizing structural properties of $P_k$-free graphs in a novel way. Specifically, we show that $P_k$-freeness can be decided in $\tilde{O}(1)$ rounds for $k=4$ in the $\mathsf{broadcast\;CONGEST}$ model, and in $\tilde{O}(n)$ rounds for $k=5$ in the $\mathsf{CONGEST}$ model, where $n$ is the number of nodes in the network and $\tilde{O}(\cdot)$ hides a $\mathrm{polylog}(n)$ factor. These results significantly improve the previous $O(n^{2-2/(3k+2)})$ upper bounds by Eden et al. (Dist.~Comp.~2022). We also construct a local certification of $P_5$-freeness with certificates of size $\tilde{O}(n)$. This is nearly optimal, given our $\Omega(n^{1-o(1)})$ lower bound on certificate size, and marks a significant advancement as no nontrivial bounds for proof-labeling schemes of $P_5$-freeness were previously known. For general $k$, we establish the first $\mathsf{CONGEST}$ lower bound, which is of the form $n^{2-1/\Theta(k)}$. The $n^{1/\Theta(k)}$ factor is unavoidable, in view of the $O(n^{2-2/(3k+2)})$ upper bound mentioned above. Additionally, our approach yields the \textit{first} superlinear lower bound on certificate size for local certification. This partially answers the conjecture on the optimal certificate size of $P_k$-freeness, asked by Bousquet et al. (arXiv:2402.12148). Finally, we propose a novel variant of the problem called ordered $P_k$ detection, and show a linear lower bound and its nontrivial connection to distributed subgraph detection.

==> induced_cycle.tex <==
\section{Quantum algorithm for induced $C_4$ detection}
Our algorithm for induced $C_4$ detection is governed by a threshold $\delta$. We say that a vertex is light iff its degree is at most $\delta$. An induced $C_4$ is light if at least one of its vertices is light, otherwise the cycle is heavy. 
\paragraph*{Detecting light cycles}
In the algorithm each light node first broadcasts its list of neighbors in $O(\delta)$ rounds. Each node $v$ then constructs, for each $(v,w)\in E$, a list $S(v,w)$ as follows:
\[
S(v,w)=\{
    w'\in V \mid \exists u\in V,\mathrm{deg}(u)\leq \delta, w'\in N(u)\backslash N(v)
\}
\]
Note that $v$ can construct $S(v,w)$ locally. For each edge $(v,w)$, $v$ and $w$ search the intersection of $S(v,w)$ and $N(w)$ using distributed quantum search. This can be done $$O(\sqrt{\mathrm{min}\{|S(v,w)|,|N(w)|\}})=O(\sqrt{n})$$ rounds. Therefore detecting light cycles requires $O(\delta + \sqrt{n})$ rounds.

 
\paragraph*{Detecting heavy cycles}
Let us now consider a fixed induced $C_4$: $(u,v),(v,w),(w,x),(x,u)\in E$ such that all nodes $u,v,w,x\in V$ are heavy. Consider that each node selects $n/\delta$ edges from the set of its incident edges uniformly at random, and broadcasts them. Then, $u$ constructs for each edge $(u,v)\in E$
\[
S(v)=\{
    x \in V \mid \exists w\notin N(u) \text{ such that }(v,w)\in E \text{ and } (w,x)\in E
\}
\]
Define the function $f_v^u:V\rightarrow \{0,1\}$ where $f_v^u(x)=1$ iff $x\in S(v)\backslash N(v)$. Using distributed quantum search, we can determine if there exists $x$ for which $f_v^u(x)=1$ using the edge $(u,v)$ in $O(\sqrt{n})$ rounds.

Since both the edges $(v,w)$, $(w,x)$ are sent to $u$ with porobability at least $1/\delta^2$, repeating this procedure $O(\delta^2)$ times we can detect heavy cycles. Furthermore, applying amplitude amplification, the number of repetition can be reduced to $O(\delta)$ times, leading to the round complexity $O\left(\left(\frac{n}{\delta} + \sqrt{n}\right)\delta\right)$.

We now consider the following protocol in which both the edges $(v,w)$, $(w,x)$ are sent to $u$ with probability at least $1/\delta$, instead of $1/\delta^2$. 

In the algorithm each node $u$ first selects an integer $\mathsf{ID}(u)$ from $[\delta]$ uniformly at random and broadcasts it to all its neighbors. Then $u$ divide $N(u)$ into $\delta$ subsets $N_i(u)$ for $i\in[\delta]$ where
$$
N_i(u) = \{
v\in N(u)\mid \mathsf{ID}(v) = i.
\}
$$
Note that $|N_i(u)|=O\left(\frac{|N(u)|}{\delta}\right) = O\left(\frac{n}{\delta}\right)$ with high probability. We thus condition on this event. Each node $u$ then selects $i\in [\delta]$ uniformly at random and asks its neighbors $v$ to send $N_i(v)$. In this procedure the edges $(v,w)$, $(w,x)$ are sent to $u$ with probability at least $1/\delta$. This leads to the round complexity $O\left(\left(\frac{n}{\delta} + \sqrt{n}\right)\sqrt{\delta}\right)$. Taking $\delta=\sqrt{n}$, we get the $O(n^{3/4})$-round algorithm for detecting induced $C_4$.
